Fantastic Multi-Task Gradient Updates and How to Find Them In a Cone

Balancing competing objectives remains a fundamental challenge in multi-task learning (MTL), primarily due to conflicting gradients across individual tasks. A common solution relies on computing a dynamic gradient update vector that balances competing tasks as optimization progresses. Building on this idea, we propose ConicGrad, a principled, scalable, and robust MTL approach formulated as a constrained optimization problem. Our method introduces an angular constraint to dynamically regulate gradient update directions, confining them within a cone centered on the reference gradient of the overall objective. By balancing task-specific gradients without over-constraining their direction or magnitude, ConicGrad effectively resolves inter-task gradient conflicts. Moreover, our framework ensures computational efficiency and scalability to high-dimensional parameter spaces. We conduct extensive experiments on standard supervised learning and reinforcement learning MTL benchmarks, and demonstrate that ConicGrad achieves state-of-the-art performance across diverse tasks.

==> files/algo_v2.tex <==
\begin{algorithm}[tb]
    \caption{\textsc{ConicGrad}}
    \label{alg:algo_2}
    \begin{algorithmic}[1]
        \STATE {\bfseries Input:} 
            Initial parameter $\theta_0$, 
            Differentiable task losses $\{l_i\}_{i=1}^{L}$, 
            Learning rates $\eta_1$ and $\eta_2$,
            Decay $\gamma$,
            Cosine similarity constraint $c$,
            Negligence coefficient $\beta$, and
            Regularization coefficient $\zeta$
        \STATE Initialize the task logits to all zeros: $z_1 = 0$
        \FOR{$t=1$ {\bfseries to} $T$}
            \STATE Compute the gradients of each loss function $\nabla_\theta l_i$
            \STATE Compute the naive gradient $g_0 = \sum_{i=1}^{L} \nabla_\theta l_i$
            \STATE Compute $\omega_t = \textrm{Softmax}(z_t)$
            \STATE Compute the weighted gradient $g_\omega = \sum_{i=1}^{L} \omega_i \nabla_\theta l_i$
            \STATE Set $b = g_\omega + c \norm{g_0}^2 g_0$ and $M = e \norm{a}^2 I + a a^T$, and compute $d^* = M^{-1} b$ following Sections~\ref{sec:smw} and \ref{sec:mul}
            \STATE Compute $\tilde{d}$ following~\cref{eq:norm}
            \STATE Formulate the auxiliary loss following \cref{eq:final_opt}
            \STATE Take an optimization step towards updating the logits $z$ using the learning rate $\eta_2$
            \STATE Compute $\omega_{t+1} = \textrm{Softmax}(z_{t+1})$
            \STATE Recompute $\tilde{d}$ based on the optimized weights $\omega_{t+1}$
            \STATE Update the model parameters $\theta_{t+1} = \theta_t - \eta_1 \tilde{d}$
        \ENDFOR
    \end{algorithmic}
\end{algorithm}

% \begin{algorithm}[tb]
%     \caption{\textsc{ConicGrad}}
%     \label{alg:algo}
%     \begin{algorithmic}[1]
%         \STATE {\bfseries Input:} 
%             Initial parameter $\theta_0$, 
%             Differentiable task losses $\{l_i\}_{i=1}^{L}$, 
%             Learning rates $\eta_1$ and $\eta_2$,
%             Decay $\gamma$,
%             Cosine similarity constraint $c$,
%             Negligence coefficient $\beta$, and
%             Regularization coefficient $\zeta$
%         \STATE Initialize the task logits to all zeros: $z_1 = 0$
%         \FOR{$t=1$ {\bfseries to} $T$}
%             \STATE Compute the gradients of each loss function $\nabla_\theta l_i$
%             \STATE Compute the naive gradient $g_0 = \sum_{i=1}^{L} \nabla_\theta l_i$
%             \STATE Compute $\omega_t = \textrm{Softmax}(z_t)$
%             \STATE Compute the weighted gradient $g_\omega = \sum_{i=1}^{L} \omega_i \nabla_\theta l_i$
%             \STATE Set $b = g_\omega + c \norm{g_0}^2 g_0$ and $M = e \norm{a}^2 I + a a^T$, and compute $d^* = M^{-1} b$ following Sections~\ref{sec:smw} and \ref{sec:mul}
%             \STATE Compute $\tilde{d}$ as $\tilde{d} = d^* \frac{\norm{g_0}}{\norm{d^*}}$
%                 \COMMENT ~\Cref{eq:norm}
%             \STATE Formulate the auxiliary loss following \cref{eq:final_opt}
%             \STATE Take an optimization step towards updating the logits $z$ using the learning rate $\eta_2$
%             \STATE Compute $\omega_{t+1} = \textrm{Softmax}(z_{t+1})$
%             \STATE Recompute $\tilde{d}$ based on the optimized weights $\omega_{t+1}$
%             \STATE Update the model parameters $\theta_{t+1} = \theta_t - \eta_1 \tilde{d}$
%         \ENDFOR
%     \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[tb]
%     \caption{Bubble Sort}
%     \label{alg:example}
%     \begin{algorithmic}
%         \STATE {\bfseries Input:} data $x_i$, size $m$
%         \REPEAT
%         \STATE Initialize $noChange = true$.
%         \FOR{$i=1$ {\bfseries to} $m-1$}
%         \IF{$x_i > x_{i+1}$}
%         \STATE Swap $x_i$ and $x_{i+1}$
%         \STATE $noChange = false$
%         \ENDIF
%         \ENDFOR
%         \UNTIL{$noChange$ is $true$}
%     \end{algorithmic}
% \end{algorithm}


==> files/fig_geometry.tex <==
\begin{figure*}[t]
    \footnotesize
    \centering
    % Subfigure 1
    \subfigure[\(d=\frac{1}{2} (g_1+g_2)\)]{
        \centering
        \includegraphics[width=0.175\textwidth]{imgs/gd.png}
        \label{fig:sub1}
    }
    \hfill
    % Subfigure 2
    \subfigure[
        \begin{equation*}
            \begin{aligned}
                \max_{d} & \min_{i} \ g_i^\top d \\
                \text{s.t.} \; & \norm{d} \leq 1
            \end{aligned}
        \end{equation*}
    ]{
        \centering
        \includegraphics[width=0.175\textwidth]{imgs/mgda.png}
        \label{fig:sub2} 
    }
    \hfill
    % Subfigure 3
    \subfigure[
        \begin{equation*}
            \begin{aligned}
                d = & \frac{1}{2} (g_{1 \perp 2} + g_{2 \perp 1})\\
                \text{where} \; & g_{i \perp j} = g_i - \frac{g_i^\top g_j}{\norm{g_j}} g_j
            \end{aligned}
        \end{equation*}
    ]{
        \centering
        \includegraphics[width=0.175\textwidth]{imgs/pcgrad.png}
        \label{fig:sub3}
    }
    \hfill
    % Subfigure 4
    \subfigure[Caption for Subfigure 4]{
        \centering
        \includegraphics[width=0.175\textwidth]{imgs/cagrad.png}
        \label{fig:sub4}
    }
    \hfill
    % Subfigure 5
    \subfigure[Caption for Subfigure 5]{
        \centering
        \includegraphics[width=0.195\textwidth]{imgs/conicgrad.png}
        \label{fig:sub5}
    }
    \caption{Main caption for the figure containing five subfigures. Subcaptions are now truly centered.}
    \label{fig:main}
\end{figure*}

==> files/table_qm9.tex <==
\begin{table*}[!t]
\centering
\caption{\textbf{Results on QM-9 dataset (11 tasks).} We repeat each experiment over \(3\) different seeds and report the average results. \(\textbf{MR}\) and \textbf{\(\Delta\) m\%} are main MTL metrics.}
\label{tab:qm9}
\scalebox{0.83}{
\begin{tabular}{@{}lccccccccccccc@{}}
\toprule
\multirow{2}{*}{Method} & \(\mu\) & \(\alpha\) & \(\epsilon_{\text{HOMO}}\) & \(\epsilon_{\text{LUMO}}\) & \(\langle R^{2}\rangle\) & ZPVE & \(U_{0}\) & \(U\) & \(H\) & \(G\) & \(c_{v}\) & \textbf{MR} \(\downarrow\) & \textbf{\(\Delta\) m\%} \(\downarrow\) \\ \cline{2-12}
 & \multicolumn{11}{c}{MAE \(\downarrow\)}  &  &  \\ \midrule
STL & \(0.07\) & \(0.18\) & \(60.6\) & \(53.9\) & \(0.50\) & \(4.53\) & \(58.8\) & \(64.2\) & \(63.8\) & \(66.2\) & \(0.07\) &  &  \\ 
\midrule
LS & \(0.11\) & \(0.33\) & \(73.6\) & \(89.7\) & \(5.20\) & \(14.06\) & \(143.4\) & \(144.2\) & \(144.6\) & \(140.3\) & \(0.13\) &  & \(177.6\) \\
SI & \(0.31\) & \(0.35\) & \(149.8\) & \(135.7\) & \(1.00\) & \(4.51\) & \(55.3\) & \(55.8\) & \(55.8\) & \(55.3\) & \(0.11\) &  & \(77.8\) \\
RLW~\citep{lin2021reasonable} & \(0.11\) & \(0.34\) & \(76.9\) & \(92.8\) & \(5.87\) & \(15.47\) & \(156.3\) & \(157.1\) & \(157.6\) & \(153.0\) & \(0.14\) &  & \(203.8\) \\
DWA~\citep{liu2019end} & \(0.11\) & \(0.33\) & \(74.1\) & \(90.6\) & \(5.09\) & \(13.99\) & \(142.3\) & \(143.0\) & \(143.4\) & \(139.3\) & \(0.13\) &  & \(175.3\) \\
UW~\citep{kendall2018multi} & \(0.39\) & \(0.43\) & \(166.2\) & \(155.8\) & \(1.07\) & \(4.99\) & \(66.4\) & \(66.8\) & \(66.8\) & \(66.2\) & \(0.12\) &  & \(108.0\) \\
MGDA~\citep{sener2018multi} & \(0.22\) & \(0.37\) & \(126.8\) & \(104.6\) & \(3.23\) & \(5.69\) & \(88.4\) & \(89.4\) & \(89.3\) & \(88.0\) & \(0.12\) &  & \(120.5\) \\
PCGrad~\citep{yu2020gradient} & \(0.11\) & \(0.29\) & \(75.9\) & \(88.3\) & \(3.94\) & \(9.15\) & \(116.4\) & \(116.8\) & \(117.2\) & \(114.5\) & \(0.11\) &  & \(125.7\) \\
CAGrad~\citep{liu2021conflict} & \(0.12\) & \(0.32\) & \(83.5\) & \(94.8\) & \(3.22\) & \(6.93\) & \(114.0\) & \(114.3\) & \(114.5\) & \(112.3\) & \(0.12\) &  & \(112.8\) \\
IMTL-G~\citep{liu2021towards} & \(0.14\) & \(0.29\) & \(98.3\) & \(93.9\) & \(1.75\) & \(5.70\) & \(101.4\) & \(102.4\) & \(102.0\) & \(100.1\) & \(0.10\) &  & \(77.2\) \\
NashMTL~\cite{navon2022multi} & \(0.10\) & \(0.25\) & \(82.9\) & \(81.9\) & \(2.43\) & \(5.38\) & \(74.5\) & \(75.0\) & \(75.1\) & \(74.2\) & \(0.09\) &  & \(62.0\) \\
FAMO~\citep{NEURIPS2023_b2fe1ee8} & \(0.15\) & \(0.30\) & \(94.0\) & \(95.2\) & \(1.63\) & \(4.95\) & \(70.82\) & \(71.2\) & \(71.2\) & \(70.3\) & \(0.10\) &  & \(58.5\) \\ 
\midrule
\rowcolor{rowcolor} \textbf{\textsc{ConicGrad}} &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \bottomrule
\end{tabular}
}
\end{table*}


==> sections/old/intro_kj.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{imgs/fig01_v1.png}
    \vspace{-2em}
    \caption{\textbf{Toy Example.} 
    On left, visualization of the loss trajectories of different MTL methods for five different initialization points on a toy 2-task learning problem is plotted. 
    FAMO and NashMTL reach any point on the Pareto front (gray curve), 
    while CAGrad and \textsc{ConicGrad} reach the global minima (\(\star\)). 
    However, \textsc{ConicGrad} is much faster than CAGrad; 
    the color of trajectories range from blue to green with more green indicating later in the trajectory. 
    On right, convergence speed of MTL methods over training steps is visualized. 
    \textsc{ConicGrad} converges to the lowest loss (dotted black line) faster than all methods.}
    \label{fig:toyexample}
\end{figure*}

Several deep learning methods tend to learn some set of parameters for a single downstream task~\citep{long2015fully,he2017mask}. 
In many real-world applications, where resources are not abundant, it is natural to then consider if some part of the underlying model structure can be shared for a diverse set of tasks. 
In literature, jointly learning parameters of multiple tasks through a shared underlying model structure refers to Multi-Task Learning (MTL)~\citep{vandenhende2021multi}. 
However, learning several tasks at once requires solving a complicated optimization problem that is often not parsimonious in data, compute, and memory requirements~\citep{navon2022multi,yu2020gradient,xiao2024direction}. 
In principle, MTL is studied under two major categories: 
multi-task architecture~\citep{lin2025mtmamba,zhang2025sgw} and optimization strategies~\citep{navon2022multi,yu2020gradient,xiao2024direction,NEURIPS2023_b2fe1ee8}.

In this manuscript, we study the MTL problem under the lens of multi-objective optimization, and the goal of these methods is to dynamically re-weight all the task losses. 
A naive objective thereof is to set the average of all the task gradients as the new gradient direction, or minimize the average loss over all the tasks. 
However, in practice this often impedes the learning performance~\citep{liu2021conflict}. 
The desiderata of efficient multi-objective optimization is to consider conflicts in gradients wherein gradients of different tasks point in opposite directions (i.e., they are in conflict with each other). 
The earliest work on multi-objective optimization utilizes gradient-based optimization and converges to a point on the Pareto set~\citep{desideri2012multiple}, and an efficient implementation is proposed in~\citep{sener2018multi}. 
Another work~\citep{yu2020gradient} directly manipulates the gradients by projecting one task's gradient onto the normal plane of the other to avoid conflicts. 
A few prior works in literature attempt to impose different constraints on the update direction of the joint gradient by formulating an update vector. 
Among those, CAGrad looks for the said update vector within an Euclidean ball with average gradient at its center~\cite{liu2021conflict}, 
while SDMGrad~\cite{xiao2024direction} enforces the update direction to be within the vicinity of the target gradient direction realized through inner-product regularization. 
Different from these, FAMO~\citep{NEURIPS2023_b2fe1ee8} is an efficient method that minimizes all the task losses in constant space and time solving the log of MGDA objective~\citep{desideri2012multiple,sener2018multi}, 
but amortizing the computation in time. 
We find that while FAMO~\citep{NEURIPS2023_b2fe1ee8} is fast, 
its performance is significantly lower than NashMTL~\citep{navon2022multi} and IMTL-G~\citep{liu2021towards}. 
On the flip side, methods that score higher in multi-task performance are computationally intractable, often requiring multiple steps in order to compute the gradient update~\citep{xiao2024direction,navon2022multi,liu2021towards}. 

In this work, we revisit the multi-task learning problem from the perspective of multi-objective optimization and propose a novel approach, \textsc{ConicGrad}, that directly operates on the task gradients. 
Unlike prior methods that impose rigid constraints on gradient directions or require computationally expensive optimization steps, \textsc{ConicGrad} offers a geometric perspective by restricting the gradient update direction within a cone. 
This allows for greater flexibility in optimization and admits a larger number of direction vectors in the conic section as long as the direction vector \(d\) forms an angle of at most \(\arccos (c)\) with the preference vector. 
Figure~\ref{fig:toyexample} illustrates the advantages of \textsc{ConicGrad} in a toy two-task learning problem, highlighting both its rapid convergence in terms of number of training steps, and the ability to reach not just the Pareto front, but the global minima (denoted by \(\star\)) effectively.

% while effectively managing conflicts between task gradients.

% Our approach redefines the optimization problem by leveraging correlation constraints between the update direction and a preference vector.
% Specifically, the update direction is constrained to maintain an angle within \(\arccos c\) of the preference vector, enabling efficient conflict resolution. 
% Through this formulation, \textsc{ConicGrad} ensures efficient convergence while balancing computational cost and performance across tasks.




==> sections/old/lambda_opt.tex <==
\subsection{Optimizing for \(\lambda\)}
\label{app:lambda_opt}

To optimize \(\lambda\), we first substitute \(d^*\) from \cref{eq:dstar} into \cref{eq:obj_without_max}.  
To simplify the resulting expression, 
we define \(Z \coloneqq \left(c^{2}\norm{g_{0}}^{2}\mathbb{I} - g_{0}g_{0}^\top\right)\), 
which is independent of \(\lambda\), following a similar approach as in \cref{sec:smw}.

\[
E(\lambda)\;=\;\frac{1}{\lambda}\,\bigl(g_{w}^{\top} Z^{-1}\,g_{w}\bigr)\;-\;\frac{\lambda}{2}\,\Bigl(\,c^{2}\,\|g_{0}\|^{2}\,\Bigl\|\tfrac{Z^{-1}\,g_{w}}{\lambda}\Bigr\|^{2}\;-\;\Bigl\|\tfrac{g_{0}^{\top}Z^{-1}\,g_{w}}{\lambda}\Bigr\|^{2}\Bigr).
\]

This further simplifies to

\[
E(\lambda) 
\;=\;
\underbrace{\frac{g_{w}^{\top}Z^{-1}\,g_{w}}{\lambda}}_{\text{Term 1}}
\;-\;
\underbrace{\frac{1}{2\,\lambda}
\Bigl[
   c^{2}\,\|g_{0}\|^{2}\,\|Z^{-1}\,g_{w}\|^{2} 
   - 
   \bigl(g_{0}^{\top}Z^{-1}\,g_{w}\bigr)^{2}
\Bigr]}_{\text{Term 2}}
\;=\;
\frac{1}{\lambda}\,\Bigl[
  g_{w}^{\top}Z^{-1}\,g_{w}
  \;-\;
  \tfrac{1}{2}\,
  \bigl(
    c^{2}\,\|g_{0}\|^{2}\,\|Z^{-1}\,g_{w}\|^{2}
    -
    (g_{0}^{\top}Z^{-1}\,g_{w})^{2}
  \bigr)
\Bigr].
\]

\paragraph{Derivative w.r.t. \(\lambda\)}

Define the constant part (independent of \(\lambda\)):

\[
C 
\;=\;
g_{w}^{\top}Z^{-1}\,g_{w}
\;-\;
\tfrac{1}{2}\,
\Bigl[
  c^{2}\,\|g_{0}\|^{2}\,\|Z^{-1}\,g_{w}\|^{2}
  - 
  (g_{0}^{\top}Z^{-1}\,g_{w})^{2}
\Bigr].
\]

So \(E(\lambda) \;=\; \frac{C}{\lambda}\).
Its derivative is
\[
\frac{d}{d\lambda}\,E(\lambda)
\;=\;
\frac{d}{d\lambda}\Bigl(\tfrac{C}{\lambda}\Bigr)
\;=\;
C \,\cdot \frac{d}{d\lambda}\Bigl(\tfrac{1}{\lambda}\Bigr)
\;=\;
-\frac{C}{\lambda^{2}}.
\]
However, since \(C \neq 0\), no finite \(\lambda\) satisfies the stationary condition.  

This exemplifies why, in Machine Learning (ML), iterative optimization is often preferred over algebraic closed-form solutions,
as many Lagrange-like formulations do not yield a single closed-form multiplier.  

Thus, in this work, we set \(\lambda = 1\) and found it to perform well empirically.

==> sections/old/method_v2.tex <==
\section{Mutli-Task Learning with \textsc{ConicGrad}}
\label{sec:method}
Consider the MOO objective in~\cref{eq:mooobj}, as opposed to direction-oriented constraints, we argue that correlation constraints allow greater flexibility in finding the update vector. Geometrically, we propose to restrict the gradient update direction in a cone such that the angle between the update vector \(d\) and preference vector \(g_{0}\) is at most \(\arccos{(c)}\). We can formulate this as the following optimization problem
\begin{equation}
\label{eq:org_eq}
    \max\limits_{d \in \mathbb{R}^{M}} \min\limits_{i \in [K]} \langle g_{i},d\rangle \quad s.t. \quad \frac{\langle g_{0}, d\rangle}{\norm{g_0} \norm{d}} > c,
\end{equation}
where \(d\) is the sought-after gradient update direction and \(c \in [-1,1]\), though in practice we restrict \(c \in (0,1]\) to avoid negative correlation.
% , $g_0, g_1,\dots,g_T \in \mathbb{R}^K$, $g_i{}_{[i=1..T]}$ is the gradient of the $i^{\textrm{th}}$ loss term in our objective, and $g_0 = \sum_{i=1}^{T}{g_i}$ (i.e., the naive, uniformly weighted objective).

We can re-write the constraint from~\cref{eq:org_eq} as
\begin{equation}
    c \norm{g_0} \norm{d} - \langle g_{0},d\rangle < 0.
\end{equation}
Note that \(\min\limits_{i \in [K]} \langle g_{i},d\rangle = \min\limits_{\omega \in \mathcal{W}} \langle g_{\omega},d\rangle\), where \(g_{\omega} = \sum_{i=1}^T \omega_{i} g_{i}\), and \(\omega\) is on the probability simplex, i.e., \(\forall i \quad \omega_{i} > 0\) and \(\sum_{i=1}^T \omega_{i} = 1\).
The Lagrangian of the objective in~\cref{eq:org_eq} is
\begin{equation}
\label{eq:primal}
    \max\limits_{d \in \mathbb{R}^K} \min_{\substack{\lambda \ge 0 \\ \omega \in \mathcal{W}}} g_\omega^\top d - \frac{\lambda}{2} (c \norm{g_0} \norm{d} - g_0^\top d)^2.
\end{equation}
The objective for \(d\) is concave, although with linear constraints, we find that when \(c < 1\) Slater condition holds (see proof in~\cref{appxprop:slatercond}), and we get strong duality since the duality gap is \(0\), and swap the \( \max \) and \( \min \) operators.

\begin{proposition}[Dual Objective] The dual objective of the primal problem in~\cref{eq:primal} is
\begin{equation}
\label{eq:obj}
    \min_{\substack{\lambda \ge 0 \\ \omega \in \mathcal{W}}} \max\limits_{d \in \mathbb{R}^K} g_\omega^\top d - \frac{\lambda}{2} (c \norm{g_0} \norm{d} - g_0^\top d)^2.
\end{equation}
\end{proposition}

For brevity we defer the derivation of optimal \(d^{*}\) to~\cref{appxderiv:proofsconicgrad}. However, the optimal update direction \(d^{*}\) is
\begin{equation}
\label{eq:dstar}
    d^{*} = \big((c^2 - c c')\norm{g_0}^2\mathbb{I} + g_0 g_0^\top \big)^{-1} (g_{\omega} + c \norm{g_0}^2 g_0),
\end{equation}
where $c'$ is the cosine of the actual angle between \(g_0\) and \(d\) (a hyperparameter which we know must be \(\geq c\)) and \(\mathbb{I}\) is \(M \times M\) identity matrix. \cref{eq:dstar} gives a closed form solution to compute \(d^{*}\) based on \(g_0\) and \(g_\omega\).

We arrive at~\cref{eq:dstar} by assuming the Lagrangian multiplier is \(\lambda = 1\). This can be also be searched or optimized, however for the sake of simplicity, we set it to \(\lambda = 1\) as any choice where \(\lambda \ge 0\) is valid. We validate this design choice empirically. The objective to optimize (\cref{eq:obj}) is now only dependent on \(\omega \in \mathcal{W}\), since we know \(d^{*}\) we drop \(\max\), and can be written as
\begin{equation}
\label{eq:obj2opt}
    \min_{\omega \in \mathcal{W}} g_{w}^\top d^{*} - \frac{1}{2}\left(c\norm{g_{0}}\norm{d^{*}} - \norm{g_{0}^\top d^{*}}\right)^{2}.
\end{equation}

% let \(\mathbf{A}\) denote \((c^2 - c c')\norm{g_0}^2 I + g_0 g_0^\top\) and \(\mathbf{b}\) denote \(g_\omega + c \norm{g_0}^2 g_0\), and~\cref{eq:dstar} then becomes \(d^{*} = \mathbf{A}^{-1}\mathbf{b}\).

\paragraph{Normalization for Stability.} To ensure that \(d^{*}\) remains stable, we multiply \(d^{*}\) with \(\frac{\norm{g_{0}}}{\norm{d^{*}}}\) such that the norm of \(d^{*}\) equals that of \(g_{0}\). Let \(\Tilde{d}\) denote the final gradient update vector, then we can say
\begin{equation}
    \label{eq:gradupdt}
    \Tilde{d} = d^{*}\frac{\norm{g_{0}}}{\norm{d^{*}}}.
\end{equation}
We explicitly enforce the above mentioned norm equality, i.e., \(\norm{d^{*}} = \norm{g_{0}}\), by adding a constraint controlled by a coefficient \(\zeta\) to~\cref{eq:obj2opt} and replace \(d^{*}\) with \(\Tilde{d}\) as
\begin{equation}
    \label{eq:opteqfinal}
    \min_{\omega \in \mathcal{W}} g_{w}^\top \Tilde{d} - \frac{1}{2}\left(c\norm{g_{0}}\norm{\Tilde{d}} - \norm{g_{0}^\top \Tilde{d}}\right)^{2} + \zeta\left(\norm{d^{*}} - \norm{g_{0}}\right)^{2}.
\end{equation}

\cref{eq:opteqfinal} is a well-shaped optimization problem and can be solved by using any optimization algorithm to derive \(\omega\). Once the optimal \(\omega\) is found (or, in an iterative optimization scenario, a step towards optimal \(\omega\) is taken), we can reuse~\cref{eq:dstar} to derive the gradient update with the updated \(g_{\omega}\). 


% Now, let's take a closer look at the Lagrangian:
% \begin{equation}
% \label{eq:main_cons}
% \begin{split}
%     &(c \norm{g_0} \norm{d} - g_0^\top d)^2 \\
%     &= c^2 \norm{g_0}^2 d^\top d + d^\top g_0 g_0^\top d - 2 c \norm{g_0} \norm{d} g_0^\top d
% \end{split}
% \end{equation}

% We now take the derivative with respect to $d$:
% \begin{equation}
% \label{eq:der_wrt_d}
%     g_\omega - \lambda \left[c^2 \norm{g_0}^2 d + g_0 g_0^\top d - c \norm{g_0} \big(\norm{d} g_0 + \frac{g_0^\top d}{\norm{d}} d \big) \right] = 0
% \end{equation}
% To simplify the equation and to ensure stability, 
% we enforce $ \norm{d} = \norm{g_0} $ and apply it in the third term.
% We also rewrite the forth term as follows:
% \begin{equation}
%     \frac{g_0^\top d}{\norm{d}} d = \frac{g_0^\top d}{\norm{d} \norm{g_0}} \norm{g_0} d = c' \norm{g_0} d
% \end{equation}
% where $c'$ is the cosine of the actual angle between $g_0$ and $d$ (a hyperparameter which we know must be $\geq c$).
% Now, $d^*$ becomes:
% \begin{equation}
%     d^* = \frac{\big((c^2 - c c')\norm{g_0}^2 I + g_0 g_0^\top \big)^{-1}}{\lambda} (g_\omega + \lambda c \norm{g_0}^2 g_0)
% \end{equation}
% We set $\lambda=1$ and the $d^*$ is simplified to:
% \begin{equation}
% \label{eq:dstar}
%     d^* = \big((c^2 - c c')\norm{g_0}^2 I + g_0 g_0^\top \big)^{-1} (g_\omega + c \norm{g_0}^2 g_0)
% \end{equation}
% For brevity, we represent $(c^2 - c c')\norm{g_0}^2 I + g_0 g_0^\top$ with $M$ and $g_\omega + c \norm{g_0}^2 g_0$ by $b$ hereafter.
% Eq.~(\ref{eq:dstar}) gives a closed form solution to compute $d^*$ based on $g_0$ and $g_\omega$.
% Both $g_0$ and $g_\omega$ are $K \times 1$ vectors, and $M$ is a $K \times K$ matrix. 
% Note that $M$ is a huge matrix (number of parameters squared) and inverting it is not practical. 
% However, due to it's specific structure, we can use the Sherman-Morrison-Woodbury formula to reformulate it as a $ 1 \times 1 $ (i.e., scalar) inversion instead (see Sec.~\ref{sec:smw}).

% As mentioned earlier under Eq.~(\ref{eq:der_wrt_d}), 
% we multiply $d^*$ with $\frac{\norm{g_0}}{\norm{d^*}}$ such that its norm is equal to $g_0$'s.
% As such, we obtain the final gradient update $\tilde{d}$ as follows:
% \begin{equation}
% \label{eq:norm}
%     \tilde{d} = d^* \frac{\norm{g_0}}{\norm{d^*}}
% \end{equation}

% Now, we replace $d$ with $\tilde{d}$ in Eq.~(\ref{eq:obj})
% to which we add the constraint $ \norm{d^*} = \norm{g_0} $ that needs to be also enforced, with a coefficient $\zeta$.
% \begin{equation}
% \label{eq:final_opt}
%     \min_{\substack{\omega \in \mathcal{W}}} g_\omega^\top \tilde{d} - 
%     \frac{1}{2} (c^2\norm{g_0}^2 \norm{\tilde{d}} - \norm{g_0^\top \tilde{d}})^2 + \zeta (\norm{d^*} - \norm{g_0})^2
% \end{equation}

% Eq.~(\ref{eq:final_opt}) is a well-shaped optimization problem and can be solved using any optimization algorithm to derive $\omega$. 
% Once the optimal $\omega$ is found (or, in an iterative optimization scenario, a step towards optimal $\omega$ is taken), 
% we can reuse Eq.~(\ref{eq:dstar}) to derive the gradient update with the updated $g_\omega$. 


\subsection{Efficient Computation}
\label{sec:smw}
In~\cref{eq:opteqfinal} there is the term \(\big((c^2 - c c')\norm{g_0}^2 I + g_0 g_0^\top \big)^{-1}\) which is an \(M\times M\) matrix and computing it is computationally intractable due to the inverse. However, due to it's specific structure, we can use the Sherman-Morrison-Woodbury formula~\citep{higham2002accuracy} to reformulate it as a \(1\times 1\) (i.e., scalar) inversion instead. In~\cref{eq:dstar}, let \(\mathbf{A}\) denote \((c^2 - c c')\norm{g_0}^2 I + g_0 g_0^\top\) and \(\mathbf{b}\) denote \(g_\omega + c \norm{g_0}^2 g_0\). Let \(e\) denote \(c^2 - c c'\), \(a\) denote \(g_0\), we can then re-write \(\mathbf{A}\) as

% In~\cref{eq:dstar}, let \(\mathbf{A}\) denote \((c^2 - c c')\norm{g_0}^2 I + g_0 g_0^\top\) and \(\mathbf{b}\) denote \(g_\omega + c \norm{g_0}^2 g_0\). Both \(g_0\) and \(g_\omega\) are $M \times 1$ vectors, and \(\mathbf{A}\) is a \(M\times M\) matrix. Note that \(\mathbf{A}\) is a huge matrix (number of parameters squared) and inverting it is computationally intractable. However, due to it's specific structure, we can use the Sherman-Morrison-Woodbury formula~\citep{higham2002accuracy} to reformulate it as a \(1\times 1\) (i.e., scalar) inversion instead and compute \(\mathbf{A}^{-1} \mathbf{b}\). From~\cref{eq:dstar}, we can say
\begin{equation}
\label{eq:simp_A}
    \mathbf{A} = e \norm{a}^{2}\mathbb{I} + aa^T,
\end{equation}

% We want to compute $A^{-1} b$, where $ A$ is a $ M \times M$ matrix:
% \begin{equation}
%     M = e \norm{a}^2 I + a a^T,
% \end{equation}
where \(a \in \mathbb{R}^{M \times L}\) with \(L \ll M\), \(\mathbb{I}\) is the \(M \times M\) identity matrix, \(e\) is a scalar, and \(\mathbf{b}\) is a \(M\times 1\) vector.
% To do so, we first need to compute the inverse of the matrix  $ M $.
% Given the structure of $ M $, the challenge lies in efficiently handling this expression without explicitly inverting a $ K \times K $ matrix. 
Note that the term \(a a^T\) is rank \(L\) since \(a \in \mathbb{R}^{M \times L}\). Moreover, \(M\) can be interpreted as a rank \(L\) perturbation of a scaled identity matrix \(e \|a\|^2 \mathbb{I}\). Such matrices are well-suited for the Sherman-Morrison-Woodbury formula (or matrix inversion lemma), which efficiently handles inverses of low-rank updates to diagonal matrices. Applying the matrix inversion lemma, we re-write \(\mathbf{A}^{-1} \mathbf{b}\) as
\begin{align}
\label{eq:efficientinverse}
    &\mathbf{A}^{-1} \mathbf{b} = \frac{1}{e \|a\|^2} \mathbf{b} - \frac{1}{e^2 \|a\|^4} a w, \\
    &\implies d^{*} = \frac{1}{e \|a\|^2} \mathbf{b} - \frac{1}{e^2 \|a\|^4} a w.
\end{align}
In~\cref{appxderiv:swmproof}, we detail how matrix inversion lemma is applied and derive~\cref{eq:efficientinverse}. Nonetheless, this avoids directly inverting the \(M \times M\) matrix \(\mathbf{A}\) and reduces the problem to computations involving \(L \times L \) matrices, which are much more manageable. This approach is not only computationally tractable, but also numerically stable~\citep{higham2002accuracy}.

\subsection{Convergence Analysis}
We analyze the convergence property of \textsc{ConicGrad}.

\begin{theorem}
Assume individual loss functions \(L_{0}, L_{1}, \cdots L_{K}\) are differentiable on \(\mathbb{R}^{m}\) and their gradients \(\nabla L_{i}(\theta)\) are all \(L\text{-Lipschitz}\) with \(L > 0\), i.e., \(\norm{\nabla L_{i}(x) - \nabla L_{i}(y)} \leq L\norm{x - y}\) for \(i = 0,1,\cdots,K\), where \(L \in (0, \infty)\), and \(L_{0}\) is bounded from below i.e., \(L^{*}_{0} = \inf_{\theta \in \mathbb{R}^{m}} L_{0}(\theta) > -\infty\). Then, with a fixed step-size \(\alpha\) satisfying \(0 < \alpha < \frac{1}{L}\), and in case of \(-1 \leq c \leq 1\), \textsc{ConicGrad} satisfies the inequality
\begin{equation}
    \label{eq:rateconverge}
    \sum_{t=0}^{T}\norm{g_{0}(\theta)}^{2} \leq \frac{2(L_{0}(0)-L_{0}^{*})}{\alpha(2\kappa c-1)(T+1)}.
\end{equation}
\begin{proof}
The proof is provided in~\cref{appx:cagradcongvergence}.
\end{proof}
\end{theorem}
\subsection{Interpreting \textsc{ConicGrad}}
\begin{figure}
    \centering
    \scalebox{0.9}{
    \includegraphics[width=\linewidth]{imgs/cagrad_vs_conicgrad.png}
    }
    \vspace{-1em}
    \caption{\textbf{Visualizing Conic and Directional Constraints.} We visualize \textsc{ConicGrad} and CAGrad~\citep{liu2021conflict} constraints in a toy setup. The x and y axes denote all possible direction vectors in \(2D\) space \(\mathbb{R}^{2}\), and the plot indicates which vectors in this space satisfy \colorbox{conicgrad}{\textsc{ConicGrad}} and \colorbox{cagrad}{CAGrad} constraints.}
    \label{fig:interpretingconicgrad}
\end{figure}

We argue that angular constraints in our proposed approach allow more freedom in the selection of the gradient update vector (\(d\)), as opposed to the direction-oriented constraints in CAGrad~\citep{liu2021conflict}. We present a geometric interpretation of the two constraints in a toy \(2D\) vector space spanned by all the possible direction vectors. \cref{fig:interpretingconicgrad} visualizes this setup, and indicates which vectors in this space satisfy \colorbox{conicgrad}{\textsc{ConicGrad}} and \colorbox{cagrad}{CAGrad} constraints. We set \(c = 0.5\) in both cases, which means that the average gradient vector \(g_{0}\) is \((1,0)\) and the feasible region for CAGrad is a Euclidean ball of radius \(0.5\) centered at this vector. However, in the case of \textsc{ConicGrad}, the angular constraint flexibly admits a larger number of direction vectors in the conic section as long as the direction vector \(d\) forms an angle of at most \(60^\circ\) with the average gradient vector \(g_{0}\). \textsc{ConicGrad} is also interpretable given that the geometry of the constraint can be interpreted as taking a gradient step within a conic section around the preference vectors. We discuss geometric interpretation of \textsc{ConicGrad} in more detail in~\cref{appxsec:geometryconic}.





% \subsection{Sherman-Morrison-Woodbury formula}
% The Sherman-Morrison-Woodbury (SMW) formula states:
% \begin{equation}
%     (A + UCV)^{-1} = A^{-1} - A^{-1} U (C^{-1} + V A^{-1} U)^{-1} V A^{-1}.
% \end{equation}
% Here we have $ A = e \norm{a}^2 I $ (diagonal) 
% and
% $ C = 1 $, $ U = a $, and $ V = a^T $ (the low-rank term).
% To apply the formula, we follow these steps:
% \begin{enumerate}
%     \item Compute $ A^{-1} $;  
%    since $ A = e \|a\|^2 I $, its inverse is:
%    \begin{equation}
%    A^{-1} = \frac{1}{e \|a\|^2} I.
%    \end{equation}
%    \item Form $ C^{-1} + V A^{-1} U $:  
%    Substituting $ U = V = a $ and $ A^{-1} $:
%    \begin{equation}
%    I + a^T A^{-1} a = I + \frac{1}{e \|a\|^2} a^T a.
%    \end{equation}
%    This is a $ L \times L $ matrix.
%     \item Invert the smaller $ L \times L $ matrix:  
%    \begin{equation}
%    D = \left( I + \frac{1}{e \|a\|^2} a^T a \right)^{-1}.
%    \end{equation}
%    \item Construct the final inverse using SMW:
%    \begin{equation}
%    M^{-1} = \frac{1}{e \|a\|^2} I - \frac{1}{e^2 \|a\|^4} a D a^T.
%    \end{equation}
% \end{enumerate}

% \subsection{Compute $ M^{-1} b $}
% \label{sec:mul}
% Now that we have the inverse $ M^{-1} $, we can compute $ M^{-1} b $ without explicitly forming $ M^{-1} $ as follows:
% \begin{enumerate}
%     \item First compute:
%    \begin{equation}
%         v = a^T b \quad (\textrm{size:\quad} L \times 1).
%    \end{equation}
%     \item Then compute:
%    \begin{equation}
%         w = D v \quad (\textrm{size:\quad} L \times 1).
%    \end{equation}
%     \item Combine results:
%    \begin{equation}
%         M^{-1} b = \frac{1}{e \|a\|^2} b - \frac{1}{e^2 \|a\|^4} a w.
%    \end{equation}
% \end{enumerate}



\input{files/algo}

% \subsection{Approximating the second call to SMW after weight update}
% Given:
% \begin{itemize}
%     \item $ E z $ (a $ K \times 1 $ matrix)
%     \item $ z $ and $ z' $ (both $ T \times 1 $ vectors)
% \end{itemize}
% where $ E $ is a $ K \times T $ implicit matrix (i.e., not given),
% we want to compute $ E z' $ without explicitly reconstructing $ E $.
% $ E z $ contains information about how $ E $ projects $ z $ into the $ K $-dimensional space. We can use this information, together with the relationship between $ z $ and $ z' $, to approximate $ E z' $ by decomposing $ z' $ in terms of $ z $.

% \subsection{Projection Approximation}
% We assume $ z' $ lies in the subspace spanned by $ z $, scaled by a factor:
% \begin{equation}
%     z' = \alpha z + \Delta,
% \end{equation}
% where
% $ \alpha $ is a scalar coefficient that aligns $ z' $ with $ z $
% and
% $ \Delta $ is the residual orthogonal to $ z $. 
% Here, we ignore $ \Delta $, assuming $ z' $ is sufficiently aligned with $ z $.

% From this decomposition, we can approximate:
% \begin{equation}
%     E z' \approx \alpha \cdot E z2,
% \end{equation}
% where $ \alpha $ is computed as:
% \begin{equation}
%     \alpha = \frac{z'^T z}{z^T z}.
% \end{equation}
% The coefficient $\alpha$ computes the scalar projection of $z'$ onto $z$ in the $K$-dimensional space.
% This scalar measures how much of $z'$ lies in the direction of $z$, relative to the magnitude of $z$. The term $z^T z$ represents the squared norm of $z$, and $z'^T z$ is the dot product, which quantifies the alignment between $z'$ and $z$. 
% When $\alpha$ is applied to $E z$, it scales $E z$ to approximate $E z'$ under the assumption that $z'$ is primarily aligned with $z$ (i.e., $z'$ lies near the span of $z$).

% Note that this approximation is accurate if $ z' $ is close to $ z $ in terms of direction or lies primarily in the subspace spanned by $ z $. This is most likely the case, since our step size for updating the $z$ is small.
% However, if $ z' $ is orthogonal to $ z $, the method will fail, as the scaling factor $ \alpha $ will not capture the contribution of $ \Delta $ (the orthogonal residual). In this case, additional information about $ E $ or $ \Delta $ would be needed.
